A Diver Attention Estimation Framework for Effective Underwater Human-Robot Interaction

Many underwater tasks, such as cable-and-wreckage inspection and search-and-rescue, can benefit from robust Human-Robot Interaction (HRI) capabilities. With the recent advancements in vision-based underwater HRI methods, Autonomous Underwater Vehicles (AUVs) have the capability to interact with their human partners without requiring assistance from a topside operator. However, in these methods, the AUV assumes that the diver is ready for interaction, while in reality, the diver may be distracted. In this paper, we attempt to address this problem by presenting a diver attention estimation framework for AUVs to autonomously determine the attentiveness of a diver, and developing a robot controller to allow the AUV to navigate and reorient itself with respect to the diver before initiating interaction. The core element of the framework is a deep convolutional neural network called DATT-Net. It is based on a pyramid structure that can exploit the geometric relations among 10 facial keypoints of a diver to estimate their head orientation, which we use as an indicator of attentiveness. Our on-the-bench experimental evaluations and real-world experiments during both closed- and open-water robot trials confirm the efficacy of the proposed framework.

==> data-tex/fig_keypoints_error.tex <==
\begin{figure}[t]
    \centering
    \vspace{2mm}
    \includegraphics[width=.99\linewidth]{data/kp_error.png}
    \caption{A bar plot showing the regression error for each of the $10$ facial keypoints.}
    \label{fig:kp_error}
    \vspace{-2mm}
\end{figure}
